Technologies on Effectiveness and Efficiency: A Survey of State Spaces Models

State Space Models (SSMs) have emerged as a promising alternative to the popular transformer-based models and have been increasingly gaining attention. Compared to transformers, SSMs excel at tasks with sequential data or longer contexts, demonstrating comparable performances with significant efficiency gains. In this survey, we provide a coherent and systematic overview for SSMs, including their theoretical motivations, mathematical formulations, comparison with existing model classes, and various applications. We divide the SSM series into three main sections, providing a detailed introduction to the original SSM, the structured SSM represented by S4, and the selective SSM typified by Mamba. We put an emphasis on technicality, and highlight the various key techniques introduced to address the effectiveness and efficiency of SSMs. We hope this manuscript serves as an introduction for researchers to explore the theoretical foundations of SSMs.

==> sections/2_ssm_old.tex <==
% \subsection{Original Continuous SSM}
\subsection{{Classical Continuous-Time SSM}}

The concept of state space, along with the state space model, holds a significant historical backdrop. Notably, Kalman~\citep{kalman1960new} employs state space models to characterize linear dynamic systems and resolve the optimal estimation problem. The original state space model can be expressed as
\begin{align}
    &h'(t) = \mathbf{A}(t)h(t) + \mathbf{B}(t)x(t), 
    \label{equ: continuous ssm1}\\
    &y(t) = \mathbf{C}(t)h(t) + \mathbf{D}(t)x(t), 
    \label{equ: continuous ssm2}
\end{align}
where $x(t) \in \mathbb{R}^{N_{\text{in}}}$ is the input vector signal, $h(t) \in \mathbb{R}^{N_{\text{s}}}$ is the state vector signal, and $y(t) \in \mathbb{R}^{N_{\text{out}}}$ is the output vector signal. $\mathbf{A}(t) \in \mathbb{R}^{N_{\text{s}} \times N_{\text{s}}}$, $\mathbf{B}(t) \in \mathbb{R}^{N_{\text{s}} \times N_{\text{in}}}$, $\mathbf{C}(t) \in \mathbb{R}^{N_{\text{out}} \times N_{\text{s}}}$, and $\mathbf{D}(t) \in \mathbb{R}^{N_{\text{out}} \times N_{\text{in}}}$ represent parameter matrices of the state space model, which are commonly referred to as the state-transition matrix, control matrix, output matrix, and direct transmission matrix respectively. 
Specifically, $\mathbf{A}(t)$ describes the time evolution of the system states, $\mathbf{B}(t)$ describes the influence of inputs on state changes, $\mathbf{C}(t)$ captures how the system states affect the output, and $\mathbf{D}(t)$ illustrates direct input-output relationships, circumventing system states.

\ybsun{add here names of matrix

A: system matrix, how the current state affects the state change x'.
B: control matrix, effect of input to change of state. 
C: output matrix, 
D: feed-forward matrix}


Generally, these parameters are either determined by the inherent characteristics of the system or acquired through conventional statistical inference methods. \ning{Add an EXAMPLE here (in physics).} \ybsun{maybe cite some works in aerospace, electrical, mechanical engineering}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/circuit.pdf}
%     \caption{The illustration of a RC oscillator circuit, where $L$, $C$, and $R$ denote the inductance, capacitance and resistance, respectively. In this system, the input signal is represented as $x(t)=[v_i(t)]$, the output signal as $y(t)=[v_o(t)]$, and the system state as $h(t)=[i_L(t), v_c(t)]^T$. The system metrices can be defined as: $\mathbf{A}(t)=\bigg[\begin{matrix}
%         -R & 0 \\
%         0 & -1
%     \end{matrix}\bigg]$, $\mathbf{C}(t)=\bigg[\begin{matrix}
%         -L\nabla_t & 0 \\
%         0 & -1
%     \end{matrix}\bigg]$, $\mathbf{B}(t)=\mathbf{D}(t)=[1]$.}
%     \label{fig:rc-oscillator}
% \end{figure}


% The original state space model operates within continuous space, where $x(t)$, $h(t)$, and $y(t)$ represent continuous signals. It is hence termed as the continuous SSM.
The above SSM described by Eq.~\ref{equ: continuous ssm1},\ref{equ: continuous ssm2} is termed as the continuous SSM because $x(t)$, $h(t)$, and $y(t)$ represent continuous signals.
\ning{Such sentences are a bit wordy,  they should be more concise, not just this case.}
This model is typically defined in the positive time domain space, which means that $t$ in Eq.~\ref{equ: continuous ssm1},\ref{equ: continuous ssm2} satisfies $t \ge 0$.
A crucial property of the continuous SSM is its linearity. Specifically, when emphasizing the input and output and simplifying ~\ref{equ: continuous ssm1},\ref{equ: continuous ssm2} to $y = \text{SSM}(\mathbf{A},\mathbf{B},\mathbf{C},\mathbf{D})(x)$, it follows that 
\begin{equation}
\text{SSM}(\mathbf{A},\mathbf{B},\mathbf{C},\mathbf{D})(x_1 + x_2) = \text{SSM}(\mathbf{A},\mathbf{B},\mathbf{C},\mathbf{D})(x_1) + \text{SSM}(\mathbf{A},\mathbf{B},\mathbf{C},\mathbf{D})(x_2).
\end{equation}

\ning{Can we use extremely simple and direct sentences to describe SSM here?}


\ning{I asked Claude, here is its version, but can be further improved:
A State Space Model (SSM) is a mathematical way to describe how systems change over time. Think of it like tracking a moving object: you need to know its current position (state) to predict where it will go next. The model uses two main equations. The first equation shows how the current state changes into the next state. The second equation shows what we can actually observe or measure from the system. SSMs are especially useful because they can handle multiple inputs and outputs at the same time. For example, when tracking a rocket, inputs might be fuel and wind speed, states might be position and velocity, and outputs might be what our sensors actually measure. Every change in the system follows clear mathematical rules, making it possible to predict future behavior or estimate hidden information from partial observations.}

The SSM is a mathematical way to describe how systems change over time.
The model works like tracking a moving object: using its current position (state) to predict where it will go next.
The SSM serves as a pivotal and versatile methodology for system description, initially finding applications in theoretical physics, communication signal processing, system control, and allied fields~\citep{findlay1904phase, bubnicki2005modern}.
SSMs are especially useful because they can handle multiple inputs and outputs at the same time. For example, when tracking a rocket, inputs might be fuel and wind speed, states might be position and velocity, and outputs might be what the sensors actually measure. Every change in the system follows clear mathematical rules, making it possible to predict future behavior or estimate hidden information from partial observations.


% \subsection{From Continuous To Discrete}
\subsection{Discretization of Continuous-Time SSMs}

\ybsun{

A good reference for discretization: https://people.sc.fsu.edu/~jpeterson/IVP.pdf

A few things to keep in mind: from differential equation to difference equation. system should bounded/lipschitz, the error goes to zero as $\Delta t \rightarrow 0$. There are some theorems in the link above if necessary,

}



In practical applications, especially when employing sequential models, the input of the system typically consists of discrete data, implying \ning{do not use ``implying'' in this case.} that the original continuous signal $x(t)$ needs to be transformed into a discrete sequence $x = (x_0, x_1, x_2, \dots)$. \ning{also too wordy}
\ning{need another example to elaborate the necessity of discretion, for example, natural languages?}
To handle such data, the state space model itself needs to undergo discretization.

In most practical applications, the SSMs are employed as sequential models. In these scenarios, the input and output of the models are discrete data $x = (x_0, x_1, x_2, \dots)$, $y = (y_0, y_1, y_2, \dots)$, instead of continuous functions $x(t)$, $y(t)$. For instance, when processing the natural language data, the input and output of the model are token embeddings, which are discrete values rather than continuous functions.
% 说明为啥连续的模型不能处理离散的数据： 





The discretization of SSMs generally involves addressing the ordinary differential equation (ODE) within the model representation, as described by Equation~\ref{equ: continuous ssm1}, and can be represented by the following equation:
\begin{align}
    &h_k = \overline{\mathbf{A}}h_{k-1} + \overline{\mathbf{B}}x_k, 
    \label{equ: discrete ssm1}\\
    &y_k = \mathbf{C}h_k + \mathbf{D}x_k,
    \label{equ: discrete ssm2}
\end{align}
where $x_k \in \mathbb{R}^{N_{\text{in}}}$, $h_k \in \mathbb{R}^{N_{\text{s}}}$, $y_k \in \mathbb{R}^{N_{\text{out}}}$, $\overline{\mathbf{A}} \in \mathbb{R}^{N_{\text{s}} \times N_{\text{s}}}$, $\overline{\mathbf{B}} \in \mathbb{R}^{N_{\text{s}} \times N_{\text{in}}}$, $\mathbf{C} \in \mathbb{R}^{N_{\text{out}} \times N_{\text{s}}}$, and $\mathbf{D} \in \mathbb{R}^{N_{\text{out}} \times N_{\text{in}}}$ have the same sizes as those in the continuous SSM.
The mathematical essence of discretizing SSMs involves expressing $\overline{\mathbf{A}}$, $\overline{\mathbf{B}}$ in terms of $\mathbf{A}$, $\mathbf{B}$, and an additional step size parameter $\Delta$. \ning{Just directly say: The key point to discretize SSMs is to representing $\overline{\mathbf{A}}$ and $\overline{\mathbf{B}}$ in terms of $\mathbf{A}$, $\mathbf{B}$, and a step size parameter $\Delta$?}
Common discretization methods include Euler’s method, zero-order hold (ZOH), and bilinear transform~\citep{gu2023modeling}:
\begin{align}
    &\textbf{(Euler)} \quad\quad \overline{\mathbf{A}} = I + \Delta \mathbf{A}, \quad\quad \overline{\mathbf{B}} = \Delta \mathbf{B}, \\
    &\textbf{(ZOH)} \quad\quad \overline{\mathbf{A}} = \text{exp}(\Delta \mathbf{A}), \quad\quad \overline{\mathbf{B}} = (\Delta \mathbf{A})^{-1}(\text{exp}(\Delta \mathbf{A}) - I)\Delta \mathbf{B}, \\
    &\textbf{(Bilinear)} \quad \overline{\mathbf{A}} = (I - \Delta \mathbf{A}/2)^{-1}(I + \Delta \mathbf{A}/2), \quad\quad \overline{\mathbf{B}} = (I - \Delta \mathbf{A}/2)^{-1}\Delta \mathbf{B}. \label{equ: Bilinear}
\end{align}
Among these three methods, Euler’s method is simple and intuitive, discretizing Equation~\ref{equ: continuous ssm1} directly as $h_k - h_{k-1} = \Delta(\mathbf{A}h_{k-1} + \mathbf{B}x_k)$, while the other two methods are more stable and accurate. 

% 或许需要添加：\Delta的具体意义，对另外2个离散化方法的解释

The discrete SSM can be utilized \ning{used, delete all the ``utilize'' in the paper.} as a sequence model to handle data that can be serialized, such as text, images, and videos. \ning{Why? Can't continuous SSM handle these?}
In contrast to the continuous SSM, the discrete SSM represents a sequence-to-sequence mapping and is often integrated as a component within larger neural network architectures, with its parameters optimized through gradient descent. \ning{need to be clear.}
It can be considered a black box that offers modeling capabilities akin to self-attention mechanisms in transformers, capturing the relationships between tokens in sequences. However, realizing its full effectiveness also necessitates additional structures such as repeated stacking and nonlinear activations.
The parameter matrix $\mathbf{D}$ of the SSM, when researched as a sequence model, is often disregarded, as it can be viewed as a skip connection, does not directly influence the state $h$, is easy to compute, and can be approximated by other structures. Consequently, Equation~\ref{equ: discrete ssm2} is commonly expressed as 
\begin{equation}
y_k = \mathbf{C}h_k. 
\label{equ: discrete ssm3}
\end{equation}
\ning{The subsection need to be clear.}

\subsection{Model Architecture Optimization}

\ning{Should be more fluent?}
Mathematically, the expression of the SSM can be derived into various forms. 
For instance, Eq.~\ref{equ: discrete ssm1},\ref{equ: discrete ssm2} naturally align with the representation format of recurrent models. \ybsun{(notations, also mention parallelizable computing)} These expressions can also lead to the derivation of convolutional forms, such as:
\begin{equation}
y = x * \overline{{\mathbf{K}} }   \quad where \quad x = (x_0, x_1, x_2, \dots),\overline{\mathbf{K}} = (\mathbf{C}\overline{\mathbf{B}}, \mathbf{C}\overline{\mathbf{AB}}, \mathbf{C}\overline{\mathbf{A}}^2\overline{\mathbf{B}}, \dots).
\label{equ: conv ssm}
\end{equation}
The diversity of SSM expressions opens up flexibility in architectural optimizations, offering a plethora of possibilities for enhancing SSM frameworks. \ning{wordy}
The vanilla SSM boasts low computational complexity and accommodates longer sequence data within equivalent computational resources, with potential acceleration through mechanisms like FFT. \ning{do not use LLMs to generate such confusing words and sentences.}
However, it is constrained by its inability to handle multi-dimensional data and instability in capturing long sequence dependencies.
In order to improve performance on tasks such as time series forecasting, long-text summarization, and two-dimensional data processing, researchers have optimized the original discrete SSM, preserving certain useful properties of the SSM while enhancing the model's capabilities in crucial aspects.


\ning{Why do we suddenly survey the recent works before introducing S4?}
To accomplish long document abstractive summarization, Bronnec et al.~\citep{bronnec2024locost} leverage the low computational complexity and superior long sequence handling offered by SSMs, constructing an encoder layer with an SSM as its central component, termed the LOCOST. Starting from the convolutional representation of SSM, they introduce the Bidirectional SSM, which incorporates causal convolution and cross-correlation to simultaneously consider contextual information before and after each token in the sequence, thus achieving improved context capture.
Baron et al.~\citep{baron20232} propose a 2-D SSM layer based on Roesser’s SSM model~\citep{givone1972multidimensional} which expands states to capture both horizontal and vertical information, thereby enhancing the SSM's understanding of two-dimensional data.
Agarwal et al.~\citep{agarwal2024spectral} apply the Spectral Filtering algorithm to learn the linear dynamical system, thereby introducing the Spectral SSM. Employing fixed spectral filters that obviate the need for learning, the model effectively maps input sequences to a new representation space and is adept at capturing long-term dependencies inherent in sequential data. These features bolster the model's prediction performance and stability, especially in sequences containing long-range dependencies.
Zhang et al.~\citep{zhang2023effectively} introduce a closed-loop prediction mechanism to SSMs, where the SSM at the decoder layer not only receives information from the encoder layer but also incorporates feedback from its own output. This design improves the flexibility and accuracy of the model in handling long-term prediction tasks.


These model structure optimizations either embed the original discrete SSM within other architectures or integrate new computational modules into the SSM structure, enhancing the performance and stability of the SSM and improving its capability to handle data with longer lengths and higher dimensions.
% Considering the constraints of limited parallelism and scalability inherent in the vanilla discrete SSM, along with its inefficient utilization of computational resources like GPUs, low training efficiency, and challenges such as exponential decay memory~\citep{wang2024state}, it is imperative to optimize the internal computational methods of SSM, which will be further detailed in subsequent sections.
However, the vanilla discrete SSM still faces several constraints, including limited parallelism, subpar scalability, inefficient training and utilization of computational resources, as well as exponential decay memory~\citep{wang2024state}. Optimizing the internal computational methods of SSMs is thus imperative, and will be further detailed in subsequent sections.
